The Kernelized Stochastic Batch Perceptron

We present a novel approach for training kernel Support Vector Machines, establish learning runtime guarantees for our method that are better then those of any other known kernelized SVM optimization approach, and show that our method works well in practice compared to existing alternatives.

==> Makefile <==
PDFLATEX = pdflatex -file-line-error -halt-on-error
LATEX = latex

FILES = \
	abstract.tex \
	app-algorithm.tex \
	app-bounds.tex \
	app-experiments.tex \
	app-generalization-bounds.tex \
	app-proofs.tex \
	app-shai.tex \
	experiments/fig-experiments.tex \
	experiments/fig-fourier-experiments.tex \
	experiments/tab-datasets.tex \
	figures/alg-slack-constrained-sgd.tex \
	figures/alg-water-bias.tex \
	figures/alg-water.tex \
	figures/fig-01-hinge-bound.tex \
	figures/fig-bias.tex \
	figures/fig-water.tex \
	figures/tab-bounds.tex \
	macros.tex \
	main.bib \
	main.tex \
	sec-algorithm.tex \
	sec-comparison.tex \
	sec-conclusion.tex \
	sec-experiments.tex \
	sec-introduction.tex \
	sec-problem.tex \
	theorems/lem-empirical-loss-from-expected-loss-proof.tex \
	theorems/lem-empirical-loss-from-expected-loss.tex \
	theorems/lem-generalization-from-empirical-loss-proof.tex \
	theorems/lem-generalization-from-empirical-loss.tex \
	theorems/lem-generalization-from-expected-loss-proof.tex \
	theorems/lem-generalization-from-expected-loss.tex \
	theorems/lem-slack-constrained-suboptimality.tex \
	theorems/lem-slack-constrained-supergradient-proof-pointer.tex \
	theorems/lem-slack-constrained-supergradient-proof.tex \
	theorems/lem-slack-constrained-supergradient.tex \
	theorems/lem-zinkevich-batch-proof-pointer.tex \
	theorems/lem-zinkevich-batch-proof.tex \
	theorems/lem-zinkevich-batch.tex \
	theorems/thm-perceptron-runtime-proof.tex \
	theorems/thm-perceptron-runtime.tex \
	theorems/thm-regularized-runtime-proof.tex \
	theorems/thm-regularized-runtime.tex \
	theorems/thm-slack-constrained-runtime-proof.tex \
	theorems/thm-slack-constrained-runtime.tex

.PHONY : all
all: main.pdf

main.pdf: $(FILES)
	$(PDFLATEX) main
	$(PDFLATEX) main
	$(PDFLATEX) main

.PHONY: clean
clean:
	rm -f main.log main.aux main.blg main.out main.pdf


==> app-generalization-bounds.tex <==
\section{SVM Generalization Bounds}\label{app:generalization-bounds}

Our goal in this section is to find a bound on the sample size $n$ required to
guarantee good generalization performance (in terms of the 0/1 loss) for a
classifier which is $\epsilon$-suboptimal in terms of the empirical hinge loss.
The bounds which we derive will be \emph{optimistic}, in the sense that they
will look like $n=O\left(\frac{1}{\epsilon^2}\right)$ when the problem is
difficult, and be better when the problem is easier, approaching
$n=O\left(\frac{1}{\epsilon}\right)$ when it is linearly separable. The main
result of this section, Lemma \ref{lem:generalization-from-expected-loss}, is a
vital building block of the bounds derived in Appendices
\ref{app:slack-constrained} and \ref{app:other-algorithms}.

In order to accomplish this, we will proceed in two stages. In the first stage
(Lemma \ref{lem:generalization-from-empirical-loss}), we will give a bound on
$n$ which guarantees good generalization performance for all classifiers which
achieve some target empirical hinge loss $L$. In the second stage (Lemma
\ref{lem:empirical-loss-from-expected-loss}), we will find a bound on $n$ which
guarantees that the empirical hinge loss is close to the expected hinge loss,
for a single arbitrary classifier. Combining these results (Lemma
\ref{lem:generalization-from-expected-loss}) will yield the sample size
required to guarantee that a suboptimal classifier is within $\epsilon$ of
the optimum.

All results in this section will be stated in the linear setting, but can (and
will) be applied equally well in the kernel setting, by applying the
transformation $x \mapsto \Phi\left(x\right)$.

We begin with the following lemma, which follows immediately from
\citet[Theorem 1]{SrebroSrTe10}:

\medskip
\input{theorems/lem-generalization-from-empirical-loss}
\input{theorems/lem-generalization-from-empirical-loss-proof}

While Lemma \ref{lem:generalization-from-empirical-loss} gives us a ``fast
rate'' on the convergence of the generalization error of classifiers with
empirical hinge loss less than the target value of $L$, the question of how to
set $L$ remains unanswered. The following lemma shows that we may take it to be
$\mathcal{L}\left( w^{*} \right) + \epsilon$, where $w^{*}$ minimizes the
expected hinge loss:

\medskip
\input{theorems/lem-empirical-loss-from-expected-loss}
\input{theorems/lem-empirical-loss-from-expected-loss-proof}

Combining lemmas \ref{lem:generalization-from-empirical-loss} and
\ref{lem:empirical-loss-from-expected-loss} gives us a bound of the desired
form, which is given by the following lemma:

\medskip
\input{theorems/lem-generalization-from-expected-loss}
\input{theorems/lem-generalization-from-expected-loss-proof}


==> figures/fig-01-hinge-bound.tex <==
\begin{figure}[t]

\centering
\includegraphics[width=0.8\columnwidth]{figures/01_hinge_bound}

\caption{
%
\small
%
Plot of a $4$-smooth and $\nicefrac{5}{4}$-bounded function which upper bounds
the 0/1 loss and lower bounds the hinge loss.
%
}

\label{fig:01-hinge-bound}

\end{figure}


==> theorems/lem-empirical-loss-from-expected-loss-proof.tex <==
\begin{proof}

The hinge loss $\ell\left(y\inner{u}{x}\right)$ is upper-bounded by
$r\norm{u}$, so $\variance[x,y]{\ell\left(y\inner{u}{x}\right)} \le
r\norm{u}\mathcal{L}\left(u\right)$. Hence, by Bernstein's inequality:
%
\begin{align*}
%
\MoveEqLeft \probability{ \hat{\mathcal{L}}\left( u \right) >
\mathcal{L}\left(u\right) + \epsilon } \\
%
& \le \exp\left( - \frac{n}{r\norm{u}}\left(
\frac{\epsilon^{2}/2}{\mathcal{L}\left(u\right)+\epsilon/3} \right) \right) \\
%
& \le \exp\left( - \frac{n}{2r\norm{u}}\left(
\frac{\epsilon^{2}}{\mathcal{L}\left(u\right)+\epsilon} \right) \right)
%
\end{align*}
%
Setting the LHS to $\delta$ and solving for $n$ gives the desired result.
%
\end{proof}


==> theorems/lem-empirical-loss-from-expected-loss.tex <==
\begin{lem}
\label{lem:empirical-loss-from-expected-loss}

Consider the expected hinge loss:
%
\begin{equation*}
%
\mathcal{L}\left(w\right) =
\expectation[x,y]{\max\left(0,1-y\inner{w}{x}\right)}
%
\end{equation*}
%
Let $u$ be an arbitrary linear classifier, and suppose that we sample a
training set of size $n$, with $n$ given by the following equation, for
parameters $\epsilon>0$ and $\delta\in\left(0,1\right)$:
%
\begin{equation}
%
\label{eq:empirical-loss-from-expected-loss-bound} n = 2 \left(
\frac{\mathcal{L}\left(u\right) + \epsilon}{\epsilon} \right)
\frac{r\norm{u}\log\frac{1}{\delta}}{\epsilon}
%
\end{equation}
%
where $r \ge \norm{x}$ is an upper bound on the radius of the data. Then, with
probability $1-\delta$ over the i.i.d.~training sample $x_{i},y_{i}:i\in\left\{
1,\dots,n\right\}$, we have that:
%
\begin{equation*}
%
\hat{\mathcal{L}}\left(u\right)\le \mathcal{L}\left(u\right) + \epsilon
%
\end{equation*}
%
where $\hat{\mathcal{L}}$ is the empirical hinge loss:
%
\begin{equation*}
%
\hat{\mathcal{L}}\left(w\right) =
\frac{1}{n}\sum_{i=1}^{n}\max\left(0,1-y_{i}\inner{w}{x_{i}}\right)
%
\end{equation*}

\end{lem}


==> theorems/lem-generalization-from-empirical-loss-proof.tex <==
\begin{proof}

\input{figures/fig-01-hinge-bound}

For a \emph{smooth} loss function \citet[Theorem 1]{SrebroSrTe10} bounds the
expected loss in terms of the empirical loss, plus a factor depending on (among
other things) the sample size. Neither the 0/1 nor the hinge losses are smooth,
so we will define a smooth loss function $\phi$ which upper bounds the 0/1 loss
and lower-bounds the hinge loss:
%
\begin{equation*}
%
\phi\left(x\right)=\left\{
%
\begin{array}{lcr}
%
\nicefrac{5}{4} & \cdots & x<-\nicefrac{1}{2}\\
%
-x^{2}-x+1 & \cdots & -\nicefrac{1}{2}\le x<0\\
%
x^{3}-x^{2}-x+1 & \cdots & 0\le x<1\\
%
0 & \cdots & x\ge1
%
\end{array}
%
\right.
%
\end{equation*}
%
This function, illustrated in Figure \ref{fig:01-hinge-bound}, is $4$-smooth
and $\nicefrac{5}{4}$-bounded. If we define:
%
\begin{align*}
%
\mathcal{L}_{\phi}\left(w\right) &=
\expectation[x,y]{\phi\left(y\inner{w}{x}\right)}\\
%
\hat{\mathcal{L}_{\phi}}\left(w\right) &=
\frac{1}{n}\sum_{i=1}^{n}\phi\left(y_{i}\inner{w}{x_{i}}\right)
%
\end{align*}
%
then the aforementioned theorem gives that, with probability $1-\delta$
uniformly over all $w$ such that $\norm{w}\le B$:
%
\begin{align*}
%
\MoveEqLeft \mathcal{L}_{\phi}\left(w\right) \le \hat{\mathcal{L}}_{\phi}\left(w\right) \\
%
& + O\left( \frac{B^2 \log^3 n}{n} + \frac{\log{\frac{1}{\delta}}}{n} \right. \\
%
& \left. + \sqrt{\hat{\mathcal{L}}_{\phi}\left(w\right)}\left( \sqrt{\frac{B^2
\log^3 n}{n}} + \sqrt{\frac{\log{\frac{1}{\delta}}}{n}} \right) \right)
%
\end{align*}
%
Because $\phi$ is lower-bounded by the 0/1 loss and upper-bounded by the hinge
loss, we'll have that for all $w$ such that $\norm{w} \le B$ and
$\hat{\mathcal{L}}\left(w\right) \le L$:
%
\begin{align*}
%
\MoveEqLeft \mathcal{L}_{0/1}\left(w\right) \le L \\
%
& + O\left( \frac{B^2 \log^3 n}{n} + \frac{\log{\frac{1}{\delta}}}{n} \right.
\\
%
& \left. + \sqrt{L}\left( \sqrt{\frac{B^2 \log^3 n}{n}} +
\sqrt{\frac{\log{\frac{1}{\delta}}}{n}} \right) \right)
%
\end{align*}
%
Setting the big-$O$ expression to $\epsilon$ and solving for $n$ gives the
desired result.
%
\end{proof}


==> theorems/lem-generalization-from-empirical-loss.tex <==
\begin{lem}
\label{lem:generalization-from-empirical-loss}

Consider the expected 0/1 loss:
%
\begin{equation*}
%
\mathcal{L}_{0/1}\left(w\right) =
\expectation[x,y]{\mathbf{1}_{y\inner{w}{x}\le0}}\\
%
\end{equation*}
%
Suppose that we sample a training set of size $n$, with $n$ given by the
following equation, for parameters $L,B,\epsilon>0$ and
$\delta\in\left(0,1\right)$:
%
\begin{equation}
%
\label{eq:generalization-from-empirical-loss-bound} n = \tilde{O}\left( \left(
\frac{L}{\epsilon} \right) \frac{\left( B + \sqrt{\log\frac{1}{\delta}}
\right)^2}{\epsilon} \right)
%
\end{equation}
%
Then, with probability $1-\delta$ over the i.i.d. training sample
$x_{i},y_{i}:i\in\left\{ 1,\dots,n\right\}$, uniformly for all linear
classifiers $w$ satisfying:
%
\begin{align*}
%
\norm{w} & \le B \\
%
\hat{\mathcal{L}}\left(w\right) & \le L
%
\end{align*}
%
where $\hat{\mathcal{L}}$ is the empirical hinge loss:
%
\begin{equation*}
%
\hat{\mathcal{L}}\left(w\right) =
\frac{1}{n}\sum_{i=1}^{n}\max\left(0,1-y_{i}\inner{w}{x_{i}}\right)
%
\end{equation*}
%
we have that:
%
\begin{equation*}
%
\mathcal{L}_{0/1}\left(w\right)\le L + \epsilon
%
\end{equation*}

\end{lem}


==> theorems/lem-generalization-from-expected-loss-proof.tex <==
\begin{proof}

Lemma \ref{lem:empirical-loss-from-expected-loss} gives that
$\hat{\mathcal{L}}\left(w\right) \le \mathcal{L}\left(u\right) + 2\epsilon$
provided that Equation \ref{eq:empirical-loss-from-expected-loss-bound} is
satisfied. Taking $L = \mathcal{L}\left(u\right) + 2\epsilon$ in Lemma
\ref{lem:generalization-from-empirical-loss} gives the desired result, provided
that Equation \ref{eq:generalization-from-empirical-loss-bound} is also
satisfied. Equation \ref{eq:generalization-from-expected-loss-bound} is what
results from combining these two bounds. The fact that this argument holds with
probability $1-2\delta$, while our claim is stated with probability $1-\delta$,
is due to the fact that scaling $\delta$ by $1/2$ only changes the bound by a
constant.
%
\end{proof}


==> theorems/lem-slack-constrained-supergradient-proof-pointer.tex <==
\begin{proof}

In Appendix \ref{app:proofs}.
%
\end{proof}


==> theorems/lem-zinkevich-batch-proof-pointer.tex <==
\begin{proof}

In Appendix \ref{app:proofs}.
%
\end{proof}

